Representation via Representations: Domain Generalization via Adversarially Learned Invariant Representations

We investigate the power of censoring techniques, first developed for learning {\em fair representations}, to address domain generalization. We examine {\em adversarial} censoring techniques for learning invariant representations from multiple "studies" (or domains), where each study is drawn according to a distribution on domains. The mapping is used at test time to classify instances from a new domain. In many contexts, such as medical forecasting, domain generalization from studies in populous areas (where data are plentiful), to geographically remote populations (for which no training data exist) provides fairness of a different flavor, not anticipated in previous work on algorithmic fairness. We study an adversarial loss function for $k$ domains and precisely characterize its limiting behavior as $k$ grows, formalizing and proving the intuition, backed by experiments, that observing data from a larger number of domains helps. The limiting results are accompanied by non-asymptotic learning-theoretic bounds. Furthermore, we obtain sufficient conditions for good worst-case prediction performance of our algorithm on previously unseen domains. Finally, we decompose our mappings into two components and provide a complete characterization of invariance in terms of this decomposition. To our knowledge, our results provide the first formal guarantees of these kinds for adversarial invariant domain generalization.

==> BACKUP_intro.tex <==
\section{Introduction}
\newcommand{\etal}{{\it et al.}}
\newcommand{\RvR}{Representation via Representations}
\newcommand{\remove}[1]{}
\newcommand{\gstar}{g^*}
\newcommand{\disp}{\mathrm{dys}}
\newcommand{\mI}{\mathds{1}}






%We investigate the power of adversarial censoring techniques, first developed for learning {\em fair representations}, to address the problem of domain generalization.
%\cnote{Introductory sentence needed.}
%Our motivating examples derive from the analysis of gene expression data. 
In gene expression analysis, as well as in much of high-throughput biology analyses on human populations, variation can arise from the intrinsic biological heterogeneity of the populations being studied, or from technological differences in data acquisition. In turn both these types of variation can be shared across studies or not.  
%As noted by Garrett-Mayer et al. (2007), the fact that the determinants of both natural and technological variation differ across studies implies that study-speciﬁc eﬀects occur in most datasets.
%This gives rise to the Harvard/Stanford problem
%
%\paragraph{The Harvard/Stanford Problem, and Beyond.}
%
For example, an algorithm for predicting whether a tumor will recur, trained on data obtained from the local population via a specific data-collection and processing method at a research hospital $A$ will typically not perform equally well on data collected at a research hospital, $B$, using different data-collection techniques and serving a potentially different local population.  

Of course, $B$ can train its own algorithm. 
%
%a machine learning algorithm for learning whether a tumor will recur is given training data consisting of biological information about sample tumors and correct labels, ``will recur early'' or ``not.''  It produces a classification algorithm that is capable of accurately labeling new examples drawn from the same population as the test samples.  But an algorithm trained, say, at Stanford, on data obtained from the local population via a specific data-collection and processing method, will not necessarily work equally well on data collected from Harvard, using different data-collection techniques and serving a potentially different local population.  Of course, the population near Harvard does not {\em need} an algorithm from Stanford -- Harvard can (and does) train its own classifier on its own training data.  
%But realistically it is not possible to develop classification and prognostication algorithms in every population and redevelop them at every slight improvement in the technologies used to collect data. Also, 
%
But what of a remote population, far from any major medical center?  The ultimate goal, in the development of models with biomedical applications, is to provide accurate predictions for fully independent samples, originating from institutions and processed by laboratories that did not generate the training datasets.  How can we transfer prediction capability to a new, geographically remote, population? 

This is a problem of {\em domain generalization}, the subject of intense study for nearly two decades.
(See Section~\ref{sec:related} for a brief overview.)
Under the assumption that there is a common signal that provides a high quality predictor $\gstar$ for {\em all} populations, and given labeled training data from several populations, can this signal be learned even when it does not necessarily yield the best predictor for any given population? When does the presence of multiple training datasets improve the accuracy of this learning procedure?

A body of literature on {\em algorithmic fairness} seeks to learn a ``neutral'' representation of the data, one from which a sensitive attribute, such as religion or sex, has been removed, while still retaining enough information to train a classifier for assigning labels to elements in the new representation space~\cite{Zemel:2013wz,Louizos:2015te,Edwards:2015vn,madras2018learning}.  The intuition is that if the representation truly has obliterated the sensitive attribute, then the labeling produced by the classifier will be fair, {\it e.g.}, treat men and women in an unbiased fashion.  

Using tools developed for fair representations, we proceed from a related, but different intuition: by training on multiple, highly diverse, sub-populations, the learning algorithm is forced to discard the idiosyncratic in preference for the universal.  
%{\it e.g.},find a prediction rule based on a signal that is shared among human sub-populations.

Domain generalization to remote populations provides a different kind of fairness, not anticipated in previous work on algorithmic fairness: representation itself, {\it i.e.}, distributing the benefit of federal research dollars throughout the land.

{\color{red} PS: We have to introduce the formal setup here. Please see Section 3 for this. This section also describes the algorithm. Bring in whatever you feel is fit. We can cut  down Section 3 after that.}

\iffalse
Similar techniques have been explored for domain adaptation~\cite{JMLR:v17:15-239}.

These last three papers use adversarial neural networks.  These are networks with two parts, which we call the {\em Learner} and the {\em Adversary}.  The Learner is trying to learn a representation space $Z$ of a data universe $X$ comprising two or more subpopulations, together with a mapping $f:X \rightarrow Z$ from inputs to their representations in $Z$, and a labeling function $\ell: Z \rightarrow \{0,1\}$, so that $\ell(f(x))$ is as accurate as possible.  The Learner is also trying to foil the Adversary, who is trying to discern from $f(x)$ the subpopulation to which $x$ belongs.  Minimizing the performance of the Adversary ensures the representation $f(x)$  hides, or ``censors,'' the subpopulation from which the instance was drawn.   
%({\color{red}PS:Suggest adding ``and other information correlated with the subpopulation" or something of this sort since it isnt just the name(?)})%; at least, computational devices of the complexity of the adversary should not be able to discern this information.ind of fairness: representation, not anticipated in learning fair representations. 
\fi


\paragraph{Contributions.}
We obtain theoretical and experimental results in domain generalization via fair representation learning.

\cnote{Add introductory sentence.}
The Encoder is trying to learn a representation space $Z$ of a data universe $X$ comprising two or more subpopulations, together with a mapping $f:X \rightarrow Z$ from inputs to their representations in $Z$, and a labeling function $\ell: Z \rightarrow \{0,1\}$, so that $\ell(f(x))$ is as accurate as possible.  The Encoder is also trying to foil the Adversary, who is trying to discern from $f(x)$ the subpopulation to which $x$ belongs.  Minimizing the performance of the Adversary ensures the representation $f(x)$  hides, or ``censors,'' the subpopulation from which the instance was drawn.   


High-level overview of our contributions. {\color{red} PS: See the red-colored text at the beginning of Section 4, and bring it here with suitable edits, if you see fit}  Note that our theoretical work is in a setting in which we have a distribution on distributions, and cite the (Muandet, Balduzzi, Scholkopf) as an antecedent.
    \begin{enumerate}
        \item In addition to baby theory giving coarse bounds on what is possible, we obtain \begin{enumerate}
            \item an analysis of excess loss in a theoretical framework that explicitly models encoding and adversarial sub-networks. We obtain both asymptotic and non-asymptotic bounds.
            \item Bounds on generalization to unseen domains, the $\varepsilon$ balls;
            \item Necessary and sufficient conditions for the existence of a good invariant representation mapping.  Sheds light on the loss functions, so might extend to distribution over distributions.  Lemma 3.2 in UD note gives us an analogue to JSD.
        \end{enumerate} 
        \item extensive experimental work on synthetic data with precedents in PNAS paper on genomic signatures, as well as colored MNIST, rotated MNIST, and PACS; includes comparison with DICA and IRM.
    \end{enumerate}

\subsection{Related Work}
\label{sec:related}

There are rich literatures of related work in computational learning theory, starting with the related problem of domain adaptation~\cite{BenDavid:2006ts,Ben-David2010}, and cross-study validation in biostatistics (see, {\it e.g.}, \cite{Parmigiani2004a,Garrett-Mayer2008,Meng:2016kt,DeVito:2016um,Rashid:2017ui,Patil:2018gr}. For brevity, we confine our discussion to domain generalization, although the literature even on this more specialized topic is vast and we cannot do it justice.
\textcolor{red}{PS: Lay out test at training or test time outline. And, what is closest to us. }
In the earliest, kernel-based, works on domain generalization~\cite{blanchard2011generalizing,muandet2013domain}, the learned classifier $f$ receives at test time not just a single $x$ drawn from a test distribution $D_T$, but a large, unlabeled, sample from $D_T$ together with a single additional test sample to be classified.  
To our knowledge, \cite{muandet2013domain} is the first to assume a latent distribution on domains (as we do). %{\color{red} PS: I went back to \cite{muandet2013domain} again and it seems to me that having one test sample should also work at test time. What am I missing? Lets please discuss.} 


The work on visual domain generalization \cite{khosla2012undoing} aims to explicitly learn the true “visual world” parameters, together with a collection of explicit shifts, where each shift leads to a different domain. 
The hope is that the true visual world parameters will give reasonable performance on the unobserved target domain.
%\cnote{More comprehensible now?}
Certain other works in this context rely on SVM-based learning algorithms \cite{xu2014exploiting,niu2015multi,niu2016exemplar}. 
This vein of empirical work shares our intuition that variation between domains helps to identify a signal that is common among the domains.

Multi-task autoencoders were introduced in~\cite{ghifary2015domain,ghifary2016scatter} for domain adaptation and domain generalization. {\textcolor{red}{Ps: Leave comment that scatterrequires multiple sample size in test.}}
%As in our work, \cite{ghifary2016scatter} assumes a latent distribution on domains. 
At the same time, \cite{Louizos:2015te} developed a model, based on deep variational autencoders, for domain adaptation and learning fair representations.
While~\cite{Zemel:2013wz} was the first work to leverage representation learning towards these latter goals, \cite{ghifary2015domain} seems to be the first to do so for domain generalization. Finding transferable representations has also been a central focus in meta-learning, that is, learning to learn. See \cite{tripuraneni2020provable} and the references therein for representation learning algorithms in the setting of multi-task learning, a problem different from domain generalization. In a separate direction, \cite{volpi2018generalizing} proposed algorithms for domain generalization based on adversarial data augmentation.
\cnote{Add a few words on what augmentation is?}
%learning 
%{\color{red} 
%for generalization to an unseen domain from a single training source. 
%The approach here is thus rather different from ours. 

%Learning transferable representations has become a central focus in meta-learning, that is, learning to learn. The recent work \cite{} considered multi-task linear regression and developed algorithms for learning a common set of features from multiple related tasks that can transfer to new unseen ones. Although sharing some similarities, this problem differs from that of domain generalization and these results apply under multi-task linear models. See \cite{} for earlier works studying representation learning in multi-task settings, most of which are empirical.}
%multi-task learning differs The rigorous results here rely crucially on the linearity assumption and the problem o
%considered multi-task learning regression and 

%an adversarial data augmentation approach for generalizing from a single training source to an unseen one. 
%\cnote{Others worth mentioning: Volpi et al 2018 Meta-Learning}

Three works are particularly aligned with our philosophical approach.  \cite{arjovsky2019invariant} comes from a line of work, initiated in~\cite{peters2016causal}, on causal inference and predictive robustness, relying on a notion of probabilistic invariance. (See~\cite{buhlmann2018invariance} for a survey.) 
%\cnote{Need a sentence or two on what they achieve and how.} 
\cite{arjovsky2019invariant} seeks %to estimate 
data representations that elicit predictors satisfying certain invariance properties across the domains. This is framed as a penalized risk minimization problem, which is then solved using stochastic gradient descent. The theoretical guarantees rely on linearity assumptions \cite[Theorem 8]{arjovsky2019invariant}.
%\cite{} frames this problem as a version of 
 We provide experimental results comparing their approach to our own.
 
Adversarial networks were introduced for fair representation learning in~\cite{Edwards:2015vn,madras2018learning}\footnote{Our codebase is adapted from~\cite{madras2018learning}.}  and for domain generalization in~\cite{li2018domain,li2018deep}.
%
%Li, Pan, Wang, Kot 2018: no theory, MMD-based adversarial auto-encoder, similar in spirit, introduces a Laplace prior in the hopes of encouraging transfer to new domains.   
%
\cite{li2018domain}, uses an auto-encoder, extending the maximum mean discrepancy distance to the multi-domain setting, and introduces a Laplace prior on representations to encourage domain generalization. 
\cite{li2018deep} employs an adversarial architecture very similar to ours, expanded with a subnetwork
%{\color{blue} correcting changes in $P(Y|X)$ between distributions by correcting the changes in $P(X|Y)$.} {\color{red} PS: Suggest change to ``
that seeks to minimize the discrepancy between $\mathbb{P}(X|Y)$ across the different domains,
addressing differences in base rates among the training distributions.
In addition, this work extends the basic GAN 2-player minimax argument in~\cite{NIPS2014_5423} to multiple players, and argue its equivalence to minimizing the Jensen-Shannon divergence measure of similarity among multiple distributions. Beyond these, \cite{li2018domain,li2018deep} do not provide further theoretical results.
 %   Li, Tian, Gong, Liu, Lin, Zhang, and Tao 2018: closest in intuition to our setting, explicitly addresses searching for invariance on the conditional distributions $Y|X$,  which equalized odds (in our objective function) only nudges towards. Addresses unequal base rates through normalization (although we don't think this should be necessary if we learn to map all positives to one distribution and all negatives to another; indeed, that is why we want such a mapping, even though we don't explicitly train for this). No distribution on distributions, nice definition of domain divergence for a set of domains (not really new here; a generalization from 2 distributions proposed by Lin in 1991); contains theory describing properties of the learned representation wrt to the training distributions, but no explicit discussion of assumptions under which domain generalization applies.
   






\cnote{The future work section will be moved to later, when Zhun sets up a file for it.}
\section{Future Work}
Explain why $\mathcal{H}$-diversity is too pessimistic.  

For a set $S$ of distributions, define $\gstar(S)$ to be the classifier that minimizes (over $g \in \mathcal{H}$) the maximum (over $D\in S)$ error $\mathcal{E}_{D\in S}(g)$ (the "argminimax").  Define the dystopia $\disp(S)$ to be the maximum, over $D \in S$, of the error $\mathcal{E}_D(\gstar(S))$.  

\cnote{dystopia not a great term here.}

Notice that with this view every population is equally worthy -- we {\em never} sacrifice a small or marginalized population for the sake of better accuracy overall.  

Our ideal assumption is that the dispersion of the distribution on domains is low, meaning that for $S\sim\mathcal{D}^n$ containing $n$ independent draws from $\mathcal{D}$, $\disp(S)$ is small and 
$$\Pr_{\stackrel{S\sim\mathcal{D}^n}{D \sim \mathcal{D}}}[\mathcal{E}_D(\gstar(S)) > \disp(S)+\alpha] < tiny(n,\alpha).$$

Perhaps we can define $\disp(\mathcal{D})$ as a limit as $n$ goes to infinity of the expected dispersion of a set of $n$ independent draws from $\mathcal{D}$ and argue something about conditions for convergence.

The $n$ that we need depends on some complexity measure of $\mathcal{D}$.





==> BACKUP_theory_UD.tex <==
%\newpage
%==============================================================
\section{Formal setup}\label{sec:setup}
\newcommand{\iid}{\stackrel{\mathrm{iid}}{\sim}}
%=============
%\paragraph{Data generation scheme.} 
Define $\cX\subseteq \bR^d$ to be the covariate space and $\cY=\{0,1\}$ the outcome space. Let $\sD$ denote a finite collection of probability distributions on $\cX\times\cY$, i.e.  $\sD=\{\cD^*_1,\cD^*_2,\cdots,\cD^*_N\}$, and $\sD^{\cX}$ the corresponding set of marginal distributions induced on $\cX$. With $\mu$ defined to be a probability distribution on $\sD$, the observed data arises as follows. 
 %Throughout, we will consider there are finite many distributions in the set $\sD$, i.e. $\sD=\{\cD^*_1,\cD^*_2,\cdots,\cD^*_N\}$.
Suppose $\cD_1,\cdots,\cD_k$ are sampled i.i.d.~from $\mu$---each of these will be referred to as a seen domain---subsequently an i.i.d.~sample $S_i=\{x_{i,j},y_{i,j}\}_{j=1}^{n_{i}}$ is observed from each $\cD_i$. Let $\hat{\cD}_i$ be the empirical distribution of the observations in $S_i$. For convenience, define $\cD_{1:k}$ to be the set of seen domains   $\{\cD_1,\hdots, \cD_k \}$, and assign distinct ID's $\{1,\hdots,k  \}$ to these domains. Denote $S_{1:k} $ to be short for the collection of observed samples $\{ S_!,\hdots, S_k\}$. Define $S^\cX_i:=\{x_{i,j}\}_{j=1}^{n_{i}}$ and $g(S^\cX_i):=\{g(x_{i,j})\}_{j=1}^{n_{i}}$, for any function $g$ on $\cX$. Note that   repeated sampling is possible here; for instance, we may have $\cD_1=\cD_2=\cD^*_1$. We refrain from any assumptions on the relationship between $k$ and $N$.  For any function $g$ and distribution $\cD$, we use $g(\cD)$ to denote the distribution of $g(z)$, where $z\sim\cD$. Finally, denote $\cD_u$ to be a generic distribution in $\sD$ not included among the seen domains.

In this work, we seek to develop a classifier from the observed samples $S_{1:k}$ that performs well on any distribution drawn randomly from $\sD$. To this end, we adopt an adversarial censored learning approach. Specifically, our algorithm is adapted from \cite{madras2018learning}, where it was used for the purposes of \emph{fair representation learning}. 
%described next. 


 \paragraph{Architecture} The samples $S_{1:k}$ are first passed through an encoder that produces a representation $\{\phi(S^{\cX}_i)\}_{i=1}^k$ of the input covariates. Here, $\phi$ is a representation mapping that belongs to some function class $\Phi= \{g | g: \mathbb{R}^d \rightarrow \mathbb{R}^s \}$. The output from the encoder is subsequently passed through a discriminator $\psi_k$ of the form 
$$\psi_k(\cdot)=W\zeta(\cdot) +B,$$
where $\zeta : \mathbb{R}^s \rightarrow \mathbb{R}^p $ lies in some function class  $\Upsilon$, $W\in\bR^{k\times p}$ and $B\in\bR^k$. We further denote
$$W=(w_1,w_2,\cdots,w_{k})^\top, B=(b_1,\cdots,b_k)^\top$$
where $w_i\in\bR^{p}, b_i\in \bR$.  Thus, the discriminator constitutes a base structure $\zeta$ followed by a linear transformation, and effectively maps each input in $\mathbb{R}^s$ to $k$ unnormalized weights. For each input $\phi(x_{i,j})$, the $\ell$-th entry in the normalized version of the output $\psi_k(\phi(x_{i,j})) \in \mathbb{R}^k$ should be viewed as the discriminator's guess for the probability that $x_{i,j}$  arises from the seen domain with ID $\ell$. Finally, define $\pi_k(\cdot)$ to be the operation that maps an input vector $w$ to the index of the entry with maximal weight. If multiple entries  achieve the maximal weight, $\pi_k$ randomly picks one among the corresponding indices. Simultaneously, a predictor is trained on the encoded representations $\{\phi(S^{\cX}_i)\}_{i=1}^k$ and produces labels in the outcome space. Denote the predictor class by $\cF=\{g | g: \bR^s\mapsto \cY \}$. 

\paragraph{Loss function.} The encoder, discriminator and predictor will be simultaneously trained using a loss function that constitutes two components: (a) the loss corresponding to the predictor  
$
L_{\text{pred}}(\cD_{1:k},f,\phi)  =1/k\sum_{i=1}^{k}\bP_{(x,y)\sim\cD_i}(f(\phi(x))\neq y)$, (b) the loss corresponding to the discriminator or adversary $
L_{\text{adv}}(\cD_{1:k},\phi,\psi_k)  =\sum_{i=1}^{k}\bP_{x\sim\cD^\cX_i}(\pi_k\circ\psi_k(\phi(x))=i).$ The form of these loss functions is directly inspired from \cite{madras2018learning}.
To this end, define 
\begin{equation*}
L(\cD_{1:k},f,\phi,\psi_k;\lambda)=L_{\text{pred}}(\cD_{1:k},f,\phi)+ \lambda L_{\text{adv}}(\cD_{1:k},\phi,\psi_k),
\end{equation*}
where $\lambda>0$ is a tuning parameter, and the corresponding empirical version 
\begin{equation}\label{eq:empirical_loss}
    L(S_{1:k},f,\phi,\psi_k;\lambda)=\frac{1}{k}\sum_{i=1}^{k}\frac{1}{n_i}\sum_{j=1}^{n_i}\mI\{f(\phi(x_{i,j}))\neq y_{i,j}\}+\lambda\sum_{i=1}^{k}\frac{1}{n_i}\sum_{j=1}^{n_i} \mI\{\pi_k\circ\psi_k(\phi(x_{i,j}))=i\},
    \end{equation}
where $\mI$ is the indicator function. We seek to optimize the aforementioned loss to obtain
\begin{equation}\label{eq:optimization}
(\hat{f}_\lambda,\hat{\phi}_\lambda)=\arg \inf_{f\in\cF,\phi\in\Phi}\sup_{\psi_k\in\Psi_k}L(S_{1:k},f,\phi,\psi_k;\lambda).
\end{equation}
The infimum aims to maximize accuracy of the predictor, whereas the supremum ensures the performance of the discriminator is minimized. The final predictor for any test datapoint $x \sim \cD$ where $\cD \sim \mu$, is then given by 
 $\hat{y} := \hat{f}_{\lambda}(\hat{\phi}_\lambda (x))$. For simplicity, throughout the paper,  we only consider function classes for which the infimum and supremum can be achieved, and therefore replace $\inf$, $\sup$ in \eqref{eq:optimization} by $\min$, $\max$ respectively. In our later experiments, the function classes $\cF, \Phi, \Psi_k$ are taken to be neural nets with specific architectures. 
 
 %----------------
 {\color{red} \begin{remark}
We here explain why we choose $L_{\text{adv}}(\cD_{1:k},\phi,\psi_k)$ in that specific form and make connections to $\cH$-divergence, which is a frequently used divergence in $L_{\text{adv}}$ for invariant representation learning over two seen domains such as in \cite{madras2018learning}
\end{remark}} 
%{\color{red} PS: I do not see at the moment why this comment is here. If it stays, we need to explain properly. I will omit looking at this for now. }
 
 
 \section{Theoretical Results}

{\color{red} We proceed to build a theoretical framework for the proposed adversarial censored learning approach. Section \ref{sec:learning} provides a learning-theoretic analysis, starting with an in-depth inspection of the limiting behavior of the adversarial loss function $L_{\mathrm{adv}}$ for diverging $k$. A precise characterization of this limit contributes to a deeper understanding of the properties of this adversarial loss. We then  provide non-asymptotic generalization error bounds for the empirical loss  \eqref{eq:empirical_loss} around its  population counterpart---the limiting object from the prior step is central for determining the appropriate form of this population version.  We further establish consistency of the optimizers $\hat{f}_{\lambda}, \hat{\phi}_\lambda$ \eqref{eq:optimization}, in the sense that, these converge in the large sample limit to the corresponding optimizers of the population loss.
Section \ref{sec:generalize} provides a characterization of the prediction performance of our algorithm on unseen domains that lie within bounded $\mathcal{H}$ divergence of the seen ones. In a separate direction, Section \ref{sec:invariant} discusses  equivalent conditions for the existence of an invariant representation mapping between the seen domains.} 

%{\color{red} Ps: The above may go earlier in the Contributions section under Introduction.}

%Firstly, we demonstrate a generalization error analysis of $L(S_{1:k},f,\phi,\psi_k)$, in which we prove what is the limit when we allow both the sample size in each $S_i$ and the number of seen domains $k$ go to infinity and provide a non-asymptotic bound for the convergence rate. By that, we further establish a universal convergence analysis of our algorithms. Secondly, we show under what conditions can we obtain a relative good worst case guarantee for the prediction performance of our algorithm to an unseen domain. Lastly, we shed light upon what relationship between candidate representation mapping class $\Phi$ and $k$ seen distributions $\cD_{1:k}$ can guarantee there exists a good invariant representation mapping for the $k$ seen domains.
%=================================
\subsection{Learning theoretic analysis}\label{sec:learning}
To obtain a learning theoretic analysis of $L(S_{1:k},f,\phi,\psi_k;\lambda)$, it is crucial to understand its limiting behavior when the sample sizes $n_i$ and number of seen domains $k$ diverge. It is clear that $L(S_{1:k},f,\phi,\psi_k;\lambda)$ converges to $L(\cD_{1:k},f,\phi,\psi_k;\lambda)$ when every $n_i \
\rightarrow \infty$. Furthermore, $L_{\text{pred}}(\cD_{1:k},f,\phi)$ converges to $\bE_{
\cD\sim \mu}[\bP_{(x,y)\sim\cD}(f(\phi(x))\neq y)]$ as $k \rightarrow \infty$. Thus, we focus on studying the limiting behavior of $\max_{\psi_k\in\Psi_k}L_{\text{adv}}(\cD_{1:k},\phi,\psi_k)$ when $k$ diverges. A crucial challenge in analyzing this limit is the fact that the structure of $\psi_k$ changes with growing $k$. 
{\color{red} PS:2-3 lines further comment on the proof is in order here. This is the only tricky step. }


%We now provide answers for Q1 in the introduction and provide a non-asymptotic bound for the generalization error.
%=============
\paragraph{The limiting value.} 
%While it is intuitive that $L(S_{1:k},f,\phi,\psi_k;\lambda)$ will convergence to $L(\cD_{1:k},f,\phi,\psi_k;\lambda)$ as samples $n_i\rightarrow\infty$ for all $i\in\{1,\cdots,k\}$, what will happen if  $k\rightarrow\infty$? Notice the structure of $\psi_k$ will also change along with $k$. Before building a generalization error analysis, we need to figure out what $\sup_{\psi_k\in\Psi_k}L_{\text{adv}}(\cD_{1:k},\phi,\psi_k)$ converges to as $k\rightarrow\infty$.  

Under mild conditions, we claim that $\sup_{\psi_k\in\Psi_k}L_{\text{adv}}(\cD_{1:k},\phi,\psi_k)$ will converge to a quantity that is closely related to a  generalized version of Total Variation Distance (TV). 
%==========
\begin{assumption}[Continuity] \label{assumption:nds}
Every 
$\zeta\in\Upsilon$ and $\phi\in\Phi$ is continuous almost everywhere (a.e.). Besides, for  all $
\cD^{*\cX}_i\in\sD$,$\zeta\in\Upsilon$ and $\phi\in\Phi$, the density functions corresponding to $\zeta(\phi(\
\cD^{*X}_i))$ are continuous a.e., and {\color{red} the images of all $\zeta(\phi(\
\cD^{*X}_i))$ have non-zero volume in $p$-dimensional space.}
\end{assumption}
{\color{red} PS: I removed the assumption name for now. We never use the name, so I am not sure why we need to introduce terminology unnecessarily}
Notice fully connected neural networks with ReLU activation function are continuous a.e., since ReLU activation function is  discontinuous only at $0$.
%==========
\begin{theorem}\label{thm:limit}
Suppose $\mu$ is a probability distribution supported on  a finite set of distributions $\mathcal{D}:=\{\cD^*_1,\cD^*_2,\cdots,\cD^*_N\}$, each of which is a distribution over $\mathcal{X} \times \mathcal{Y}$. Further, let $\cD_1,\cdots,\cD_{k} \iid \mu $ with corresponding study IDs $\{1, \hdots, k \}$.
Then under Assumption \ref{assumption:nds}, for any $\phi\in\Phi$ {\color{red} and $\zeta\in\Upsilon$},
\begin{equation}\label{eq:limit}
\lim_{k\rightarrow \infty}\max_{\psi_k\in\Psi_k}\sum_{i=1}^{k}\bP_{x\sim\cD^\cX_i}(\pi_k\circ\psi_k(\phi(x))=i)={\color{red}\max_{\cup_iA_i=\bR^p,A_i\cap A_j=\emptyset, \zeta\in\Upsilon}}\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\zeta(\phi(x))\in A_i).
\end{equation}
\end{theorem}
Note that on the LHS, the probabilities are taken w.r.t.~marginal covariate distributions of the seen domains $\cD^{\cX}_i$, which may contain repeats from $\mathcal{D}$. However, on the RHS, the probabilities are w.r.t.~the corresponding marginals of the distributions in $\mathcal{D}$, each of which contributes a single term to the sum. 

%We remark here while the probabilities are taken w.r.t marginal distribution of seen domains $\cD^{\cX}_i$ on the left hand side (LHS) of Eq. \ref{eq:limit}, the probabilities on right hand side (RHS) are taken w.r.t $\cD^{*\cX}_i$. While there may be repeated sampling happens on LHS,  that will not affect the RHS. 

Moving forth, we establish a relation between the limiting object from \eqref{eq:limit} and the total variation (TV) distance.  
%we investigate the limiting o we make the connection between $\max_{\cup_iA_i=\bR^p,A_i\cap A_j=\emptyset, \zeta\in\Upsilon}\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\zeta(\phi(x))\in A_i)$ and total variational distance. 
Informally, let $\hat{\zeta}=\argmax_{\zeta\in\Upsilon}\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\zeta(\phi(x))\in A_i)$ {\color{red} (for simplicity, we ignore the uniqueness issue here).} {\color{red}PS: Cant we have $\in$ here and wont it work? } Note that when $N=2,$ 
$$\max_{\cup_iA_i=\bR^p,A_i\cap A_j=\emptyset}\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\hat{\zeta}(\phi(x))\in A_i)=TV(\hat{\zeta}(\phi(\cD^{*\cX}_1)),\hat{\zeta}(\phi(\cD^{*\cX}_2)))+1.$$
{\color{red} PS: Not sure how you get here}
For $N>2$, it is not hard to see that 
$$\max_{\cup_iA_i=\bR^p,A_i\cap A_j=\emptyset, \zeta\in\Upsilon}\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\zeta(\phi(x))\in A_i)=\max_{\cup_iA_i=\bR^p,A_i\cap A_j=\emptyset}\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\hat{\zeta}(\phi(x))\in A_i)\geq 1,$$
where equality holds iff $\hat{\zeta}(\phi(\cD^{*\cX}_1))=\cdots=\hat{\zeta}(\phi(\cD^{*\cX}_k))$. 
{\color{red} PS: Intuition: For any $\phi$, on plugging in the best possible $\zeta$, the limit is minimized when these distributions are equal. So plug in the best $\phi$, that is, the one from our algorithm. Then, the encoder followed by base structure, that is the part that remains invariant t $k$---if they map inputs to same distribution, limit is minimized, and if limit is minimized, they mapped to same distribution. This quantity governs when the algorithm is successful in finding an invariant representation. But, we can only conclude this in limit of large no. of studies---in last section provide more along these lines but for any pair of distributions. Should expect that if there is invariance, algo works well when this quantity is minimized. Draw analogies to JSD/distributional variance, Scholkopf... and later along these lines, Li's }

{\color{red} Thus, the RHS can be viewed as a generalized version of total variational distance plus $1$.} {\color{red} PS: Not sure if this directly means this.}

{\color{red}PS: So far nothing seemed to prove larger number of domains help. So, is it just in terms of the non-asymptotic bounds? What if things cancel between numerator and denominator there?}

\paragraph{Non-asymptotic generalization bounds.} 
%============
%With the help of Theorem \ref{thm:limit},
We now proceed to build a generalization error bound for $L(S_{1:k},f,\phi,\psi_k;\lambda)$. To this end, a few key quantities are introduced next. Define
\begin{align}
&L(\sD,f,\phi;\lambda) \nonumber\\
&=\bE_{
\cD\sim \mu}[\bP_{(x,y)\sim\cD}(f(\phi(x))\neq y)]+{\color{red} \sup_{\cup_i A_i=\bR^p,A_i\cap A_j=\emptyset, \zeta\in\Upsilon}}\lambda\sum_{i=1}^{N}\bP_{x\sim\cD^{*\cX}_i}(\zeta(\phi(x))\in A_i).
\end{align}
% For a fixed $\lambda$, we will provide a uniform non-asymptotic bound over $\cF$ and $\Phi$
%$$\max_{f\in\cF,\phi\in\Phi}|\max_{\psi_k\in\Psi_k} L(S_{1:k},f,\phi,\psi_k;\lambda)-L(\sD,f,\phi;\lambda)|,$$
%In order to establish such a bound, we need to introduce some new concepts and notations.
%=============
\begin{definition}[Grids]\label{def:grid}
For each integer $k>0,n>0$ and real constant $B>0$, define  $G(n,B)$ to be the set
$$G(n,B)=\{I_{i_1}\times I_{i_2}\times\cdots\times I_{i_p},i_j\in\{1,\cdots,n\} \,\, \forall \,\,j\},$$
where $I_{i_j}=[-B+2(i_j-1)B/n,-B+2i_jB/n]$.
\end{definition}

{\color{red} The elements in $G(n,B)$ form a partition of  $[-B,B]^{\times p}$ and the intersection of every pair of elements has volume $0$ in $\mathbb{R}^p$.} Denote the density function of $\zeta(\phi(\cD^{*\cX}_i))$ by $\rho^{\zeta,\phi}_i(\cdot)$ and define 
$$T^{\zeta,\phi}_i:=\{z:\rho^{\zeta,\phi}_i(z)>\rho^{\zeta,\phi}_j(z),~\text{for all}~j< i~\text{and}~\rho^{\zeta,\phi}_i(z)\geq\rho^{\zeta,\phi}_j(z),~\text{for}~j\geq i\}.$$
It is easy to see that $\{T^{\zeta,\phi}_i\}_{i=1}^{N}$ form a partition of $\bR^p$. Furthermore, let
%$$M^{\zeta,\phi}_{i,1}(n,B)=\{g:g\in G(n,B),g\subseteq T^{\zeta,\phi}_i\},~$$
$$M_{i}(n,B)=\{g:g\in G(n,B),g\nsubseteq T^{\zeta,\phi}_i,g\cap T^{\zeta,\phi}_i\neq\emptyset\}.$$
%Lastly, we need the following assumptions.
%=============
\begin{assumption}
[Boundedness]
\label{assumption:ub}
There exists a constant $B_{\rho} $ and function $B(\cdot)$ s.t.~for any $\varepsilon>0$, 
$$\sup_{\zeta,\phi}\sum_{i=1}^{N}\bP_{x\sim \cD^{*\cX}_i}(\|\zeta(\phi(x))\|\geq B(\varepsilon))\leq \varepsilon \qquad \sup_{\zeta,\phi,i}\|\rho^{\zeta,\phi}_i(\cdot)\|_\infty\leq B_\rho.$$

\end{assumption}
%==========
\begin{assumption}[Bounded VC-dimensions]\label{assumption:vc}
Assume that the function classes $\Lambda=\{f\circ \phi|f\in\cF,\phi\in\Phi\}$  and $\Xi = \{\mI\{w_1^\top\zeta( \phi(x))+b_1>w_2^\top\zeta( \phi(x))+b_2\}| w_i\in \bR^p, b_i\in \bR,\zeta\in\Upsilon,\phi\in\Phi,i=1,2\}$ have VC-dimensions $\cV_{\Lambda}$ and $\cV_{\Xi}$ respectively. 
\end{assumption}
{\color{red} We remark here in Assumption \ref{assumption:vc}, the VC dimension condition on $\Xi$ is on two nodes instead of $k$.}
%==========
\begin{theorem}\label{thm:non-asymptotic bound}
Consider the setting of Theorem \ref{thm:limit} and define $G_k := \{\cD_i \in \sD : \mu(\cD_i) \geq 1/k^{1/4} \}$, $m_k :=\lfloor k^{\frac{3}{4}}-\sqrt{(k\log(|G_k|)+k^{\frac{3}{4}})/ \sqrt{2}}\rfloor$. 
%be the set of points in $\sD$ that receive mass whose probability mass are larger or equal to $1/k^{1/4}$, and let 
%\begin{align*}
%m_k=\lfloor k^{\frac{3}{4}}-\sqrt{\frac{k\log(\text{Card}(G_k))+k^{\frac{3}{4}}}{2}}\rfloor
%\end{align*}
%where $\text{Card}(G_k)$ is the cardinality of set $G_k$. 
Under Assumptions \ref{assumption:nds}-\ref{assumption:vc}, there exists a universal constant $c$, s.t.~for any $t_1,t_2>0$, w.p.~at least  $1-e^{-k^{1/4}}-\sum_{i=0}^{k-1}4e^{-n_it_1^2}-2Ne^{-2kt_2^2}$, 
\begin{align}\label{eq:na}
\begin{split}
& \max_{f\in\cF,\phi\in\Phi}|\max_{\psi_k\in\Psi_k} L(S_{1:k},f,\phi,\psi_k;\lambda)-L(\sD,f,\phi;\lambda)|
\leq 2t_1+\frac{2\lambda}{\sqrt{k}}+\max\{N-|G_k|,0\}
+N\cdot t_2\\
&+\frac{2c}{k}\sum_{i=1}^{k}\left(\sqrt{\frac{\cV_{\cC(k)}\log(\frac{n_i}{\cV_{\cC(k)}})}{n_i}}+\sqrt{\frac{\cV_{\Lambda}\log(\frac{n_i}{\cV_{\Lambda}})}{n_i}}\right)
+\frac{2\lambda B_\rho B^p(\frac{1}{\sqrt{k}})}{\lfloor m^{1/p}_k \rfloor^p } \sum_{i\in G_k}\sup_{\zeta,\phi}|M_{i}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))|\\
\end{split}
\end{align}
where $\cV_{\cC(k)}=k\cV_{\Xi}(\log(\cV_{\Xi}))^2$. 
\end{theorem}
%\zhun{add more interpretation and examples here}
{\color{red}PS: Following I will shorten significantly. }

{\color{red} Can have $k^{\alpha}$, $\alpha \in (c_1,c_2)$.}
\paragraph{Interpretation of Theorem \ref{thm:non-asymptotic bound}}
We briefly comment on the RHS of Eq.\ref{eq:na} term by term.

I. For the term 
$$\sqrt{\frac{\cV_{\cC(k)}\log(\frac{n_i}{\cV_{\cC(k)}})}{n_i}}+\sqrt{\frac{\cV_{\Lambda}\log(\frac{n_i}{\cV_{\Lambda}})}{n_i}},$$
in order to make it vanish as $k$ grows, we need $n_i$'s increase with $k$, for instance, let $\min_{i} n_i=\Omega(k\log k)$.

II. As long as $Card(G_k)=o(\exp(\sqrt{k}))$ (which would eventually happen as $k$ grows), then $m_k=\Omega(k^{3/4})$. Thus, as long as $B^p(1/\sqrt{k})\cdot  \sum_{i\in G_k}\sup_{\zeta,\phi}|M^{\zeta,\phi}_{i,2}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))| =O(k^{3/4})$, we have 
$$\frac{B_\rho B^p(\frac{1}{\sqrt{k}})}{\lfloor m^{1/p}_k \rfloor^p }\cdot \sum_{i\in G_k}\sup_{\zeta,\phi}|M^{\zeta,\phi}_{i,2}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))|$$
goes to $0$ as $k$ goes to infinity. For $B(1/\sqrt{k})$, it reveals a uniform control of all tails of distributions in $\sD$. Suppose all distributions of domains are multi-variable sub-gaussian distributions, with sub-gaussian norm all bounded by a constant $\sigma_{\max}$, then 
$$B(\frac{1}{\sqrt{k}})=O(\sqrt{\log k}).$$
Meanwhile for $\sum_{i\in G_k}\sup_{\zeta,\phi}|M^{\zeta,\phi}_{i,2}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))|$, a trivial upper bound for it is $\lfloor m^{1/p}_k \rfloor^p$. However, in most cases, when $k$ is large, each grid's volume becomes smaller and smaller, so that the union of grids in $ M^{\zeta,\phi}_{i,1}(n,B)=\{g:g\in G(n,B),g\subseteq T^{\zeta,\phi}_i\}$ can approximate $T_i$ better and better and we would expect $\sum_{i\in G_k}\sup_{\zeta,\phi}|M^{\zeta,\phi}_{i,2}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))|=o(\lfloor m^{1/p}_k \rfloor^p)$. We give a specific example here: consider there are only $2$ elements in $\sD$, $p=2$ and 
$$T_1=\{(x_1,x_2): x_1\leq c \}$$
for a constant $c$, then we know 
$$\sum_{i\in G_k}\sup_{\zeta,\phi}|M^{\zeta,\phi}_{i,2}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))|=O(\lfloor m^{1/2}_k \rfloor)$$
If we further combine the previous assumption of sub-gaussian tail control, we have 
$$\frac{B_\rho B^p(\frac{1}{\sqrt{k}})}{\lfloor m^{1/p}_k \rfloor^p }\cdot \sum_{i\in G_k}\sup_{\zeta,\phi}|M^{\zeta,\phi}_{i,2}(\lfloor m^{1/p}_k \rfloor,B(\frac{1}{\sqrt{k}}))|=O(\frac{\sqrt{\log k}}{\lfloor m^{1/2}_k \rfloor})=O(\sqrt{\log k}k^{-3/8}).$$

III. For $\max\{N-\text{Card}(G_k),0\}$ it will goes to $0$ when $k\geq N$.

\paragraph{Consistency.}
Theorem \ref{thm:non-asymptotic bound} provides conditions under which the empirical loss function, when evaluated at the estimates $(\hat{f}_\lambda, \hat{\phi}_\lambda)$, will be close to its population counterpart w.h.p. Here we seek to  establish that these estimates indeed well approximate minimizers of the population loss. Since we impose no assumption on the form of the seen domains, this is naturally hard to prove in such generality. We will therefore establish this under a curvature condition on the population loss. {\color{red} PS: How is the following result proved? I will include a transition line here.}

\begin{assumption}[Well-separation]\label{assumption:ws}
Denote $\cM^*_{\cF,\Phi}\subseteq\cF\times\Phi$ to be the set of minimizers of $L(\sD,f,\phi;\lambda)$. For a metric $dist(\cdot,\cdot)$ on the function class $\cF\times\Phi$, there exists a function $U(\cdot;\lambda):\bR\rightarrow\bR^{+}$, such that for any $\varepsilon>0$
%, and any element $\xi\in\cF\times\Phi$,
$$\inf_{\xi \in\cF\times\Phi: ~\inf_{z\in\cM^*_{\cF,\Phi}}dist(\xi,z)\geq U(\varepsilon;\lambda)}|L(\sD,\xi;\lambda)-\min_{f\in\cF,\phi\in\Phi}L(\sD,f,\phi;\lambda)|\geq \varepsilon.$$
\end{assumption}
\begin{theorem}\label{thm:minimizer}
Under Assumption \ref{assumption:nds}-\ref{assumption:ws}, almost surely,
$$\inf_{z\in\cM^*_{\cF,\Phi}}dist((\hat{f}_\lambda,\hat{\phi}_\lambda),z)\leq U(2\Gamma;\lambda),$$
where $\Gamma$ equals the RHS of \eqref{eq:na}.
\end{theorem}
{\color{red} PS: Zhun, please comment on when the RHS above will be small.}

{\color{red} General comment: I put this back in and have changed my opinion. Assumption 4.4 looks strong at first glance. However, we are in a completely non-parametric setting---no assumptions on the form of $\cD_1,\hdots,\cD_k$ and therefore, having a structural assumption on the loss function is not as strong as it originally seemed. }




%=================================
\subsection{Generalization to unseen domains}
\zhun{this part we need to reinterpret} Previous theory leverage  how our algorithm predict a newly coming domain by minimizing an expected prediction loss with a penalty on dissimilarity among the seen domains after feeding to a representation mapping. However, minimizing an expected loss cannot guarantee a good performance on an arbitrary newly coming domain from $\sD$. In this section, we study in what condition can we have a good worst case guarantee. The intuition is straightforward: if the unseen domains can be well-represented -- meaning any unseen domain is not far from at least one of the domains with relatively high probability in a certain metric. We rigorously state the above intuition as the following.
%=============
\begin{assumption}[Well-represented]\label{assumption:rep}
There exists constants $0<p_l<1$ and $\delta>0$, s.t.~for any $\cD\in\sD$ {\color{red} with $\mu(\cD) > 0$}, $\exists \cD'\in\sD$ with $\mu(\cD') \geq p_l$ and
$d_\cH(\cD,\cD')\leq\delta,$
where $\cH=\cF\times\Phi$.
\end{assumption}
{\color{red} I rephrased your previous assumption using $\mu$. We need discuss this once.}
\zhun{H divergence should be defined at Remark 2.1}
{\color{red} PS: Are we moving away from the finite support assumption here? }

{\color{red} The follo}

%==============
\begin{theorem}\label{thm:worstcase}
Under Assumption \ref{assumption:nds}, \ref{assumption:vc} and \ref{assumption:rep}, with probability at least $1-\exp(-k^2p_l^2/2)/p_l-\sum_{i=1}^{k}4e^{-n_it^2}$, for any domain $\cD_u\in\sD$ and all $f\in\cF,\phi\in\Phi$,
$$\bP_{(x,y)\sim\cD_u}(f(\phi(x))\neq y)\leq\frac{2}{p_l} \Big(\hat{\beta}(f,\phi)+t+c\sqrt{\frac{\cV_{\Lambda}\log(n_i/\cV_{\Lambda})}{n_i}}\Big)+\delta$$
where $\hat{\beta}(f,\phi)=\sum_{i=1}^{k}\sum_{j=1}^{n_i}\bI\{f(\phi(x_{i,j}))\neq y_{i,j}\}/(kn_i).$

\end{theorem}






















%=================================
\subsection{Existence of a good invariant representation mapping}










%$L_{\text{pred}}(\cD_{1:k},f,\phi)=1/k\sum_{i=1}^{k}\bP_{(x,y)\sim\cD_i}(f(\phi(x))\neq y)$ and $L_{\text{adv}}(\cD_{1:k},\phi,\psi_k)=\sum_{i=1}^{k}\bP_{x\sim\cD^\cX_i}(\pi_k\circ\psi_k(\phi(x))=i)$. 
%\begin{equation}
%L(\cD_{1:k},f,\phi,\psi_k;\lambda)=\frac{1}{k}\sum_{i=1}^{k}\bP_{(x,y)\sim\cD_i}(f(\phi(x))\neq y)+ \lambda\sum_{i=1}^{k}\bP_{x\sim\cD^\cX_i}(\pi_k\circ\psi_k(\phi(x))=i),
%\end{equation}
%where $\lambda>0$ is a tuning par Our loss function 










%{\color{red} PS: We need to explain the algorithm that we are going to study here.}






























%==============================================================


%==========
%\begin{assumption}[Non-degenerated continuity]\label{assumption:ndc}

%\end{assumption}














%=============

%=============
%\begin{assumption}[Bounded VC-dimensions]\label{assumption:vc}

%\end{assumption}




%=================================

Adversarial methods such as in~\cite{Edwards:2015vn,JMLR:v17:15-239,li2018deep,li2018domain,madras2018learning} seek a mapping from the input space to the representation space under which the images of the training domains are indistinguishable to the adversary.  In this section we provide sufficient conditions for the existence of a mapping yielding statistically close distributions.






==> rvr_broader.tex <==
%\documentclass[11pt]{article}
%\usepackage[cm]{fullpage}
%\usepackage{fontspec}\setmainfont{Georgia}
%\begin{document}

\iffalse
High-dimensional data are the norm in current biomedical research. 
Common goals in high-dimensional data analysis is the unsupervised identification of latent components or factors (e.g. to simplify the interpretation of genome-scale measurements), and the construction of classification and prognostication algorithms (e.g. to use complex biological data to guide patient management).

When training from data drawn from multiple studies, a fundamental challenge is learning how to extract shared signal for the purposes of out-of-distribution generalization. 
\fi

\section*{Broader Impact}
In gene expression analysis, as well as in much of high-throughput biology analyses on human populations, variation between studies can arise from the intrinsic biological heterogeneity of the populations being studied, or from technological differences in data acquisition. In turn both these types of variation can be shared across studies or not.  As noted in~\cite{Garrett-Mayer2008}, the fact that the determinants of both natural and technological variation differ across studies implies that study-specific effects occur in most datasets.

The ultimate goal, in the development of models with biomedical applications, is to provide accurate predictions for fully independent samples, originating from institutions and processed by laboratories that did not generate the training datasets.  How can we transfer prediction capability to a new, possibly remote, population?  %Our work suggests and investigates a general and novel strategy to develop prediction methods that incorporate replicability for unseen populations into the learning process.  

Our work forges a new path for addressing a major problem in biomedical research, where the availability of high dimensional personal-level information is opening vast opportunities for developing predictive and prognostic algorithms to support increasingly personalized medical care, but general strategies to ensure generalizability of these algorithms beyond the populations used for training are still lacking. 
%Our motivating examples derive from the analysis of gene expression data, 
While our motivating examples derive from the analysis of gene expression data in oncology, and our synthetic data experiments are modeled on procedures for
generating synthetic data that have otherwise been employed in this field~\cite{Patil:2018gr}, our concepts and tools would be applicable to most areas of biomedicine and to a broad variety of labels, including time-to-event outcomes.

We are actively pursuing biomedical applications in several directions. For example the NCI's Genomic Data Commons (GDC) Portal provides access to a variety of relevant data. The GENIE projects include somatic mutation data on a few dozens of genes from eight cancer centers (domains) with matched clinical covariates and outcomes (labels) for over 44 thousand individuals. Also on GDC are extensive high throughput biology measurements from the Cancer Genome Atlas. In a complementary example we have initiated a collaboration to explore the utility of this approach in neuroscience data, where domains are measurement instruments (domains), and unit $j$ is a time point in a voltammetry profile. 

This work -- domain generalization to unseen populations -- provides a new dimension of fairness, {\em representation of potentially small, geographically remote populations}, not anticipated in earlier work on learning fair representations.

%\end{document}

